Fixed-Parameter Algorithms for Longest Heapable Subsequence and Maximum Binary Tree

A heapable sequence is a sequence of numbers that can be arranged in a "min-heap data structure". Finding a longest heapable subsequence of a given sequence was proposed by Byers, Heeringa, Mitzenmacher, and Zervas (ANALCO 2011) as a generalization of the well-studied longest increasing subsequence problem and its complexity still remains open. An equivalent formulation of the longest heapable subsequence problem is that of finding a maximum-sized binary tree in a given permutation directed acyclic graph (permutation DAG). In this work, we study parameterized algorithms for both longest heapable subsequence as well as maximum-sized binary tree. We show the following results: 1. The longest heapable subsequence problem can be solved in $k^{O(\log{k})}n$ time, where $k$ is the number of distinct values in the input sequence. We introduce the "alphabet size" as a new parameter in the study of computational problems in permutation DAGs. Our result on longest heapable subsequence implies that the maximum-sized binary tree problem in a given permutation DAG is fixed-parameter tractable when parameterized by the alphabet size. 2. We show that the alphabet size with respect to a fixed topological ordering can be computed in polynomial time, admits a min-max relation, and has a polyhedral description. 3. We design a fixed-parameter algorithm with run-time $w^{O(w)}n$ for the maximum-sized binary tree problem in undirected graphs when parameterized by treewidth $w$. Our results make progress towards understanding the complexity of the longest heapable subsequence and maximum-sized binary tree in permutation DAGs from the perspective of parameterized algorithms. We believe that the parameter alphabet size that we introduce is likely to be useful in the context of optimization problems defined over permutation DAGs.

==> Figures/Fig_ExtendedBT.tex <==
\begin{figure}[ht]
\begin{center}
		\begin{tikzpicture}
		\node[vertex] (a1) at (1,1) {$a$}; 
		\node[vertex] (a2) at (2,2) {$b$};
		\node[rectangle, draw=black, minimum size=15pt]  (a3) at (3,1) {$e$};
		\node[rectangle, draw=black, minimum size=15pt] (a4) at (0,0) {$c$}; 
		\node[rectangle, draw=black, minimum size=15pt]  (a5) at (2,0) {$d$};
		\path [->]
		(a1) edge (a2)
		(a3) edge (a2)
		(a4) edge (a1)
		(a5) edge (a1);
		\end{tikzpicture}
	\end{center}
\caption{Given a binary tree $T$ composed of two nodes $a$ and $b$, the extended binary tree $Ext(T)$ has two internal nodes $a$ and $b$, and three new external nodes $c$, $d$, and $e$.}
\label{fig:umbrella-free}
\end{figure}
